Domain Generalization for Medical Image Analysis: A Review

Medical image analysis (MedIA) has become an essential tool in medicine and healthcare, aiding in disease diagnosis, prognosis, and treatment planning, and recent successes in deep learning (DL) have made significant contributions to its advances. However, deploying DL models for MedIA in real-world situations remains challenging due to their failure to generalize across the distributional gap between training and testing samples - a problem known as domain shift. Researchers have dedicated their efforts to developing various DL methods to adapt and perform robustly on unknown and out-of-distribution (OOD) data distributions. This article comprehensively reviews domain generalization (DG) studies specifically tailored for MedIA. We provide a holistic view of how DG techniques interact within the broader MedIA system, going beyond methodologies to consider the operational implications on the entire MedIA workflow. Specifically, we categorize DG methods into data-level, feature-level, model-level, and analysis-level methods. We show how those methods can be used in various stages of the MedIA workflow with DL equipped from data acquisition to model prediction and analysis. Furthermore, we critically analyze the strengths and weaknesses of various methods, unveiling future research opportunities.

==> macros.tex <==
\usetikzlibrary{decorations.pathreplacing,calligraphy}
\usetikzlibrary{arrows.meta,shapes,positioning,shadows,trees}
\usetikzlibrary{shadows.blur}

\newcommand{\etal}{\textit{et~al}.\xspace}
\newcommand{\ie}{\textit{i}.\textit{e}.\xspace}
\newcommand{\eg}{\textit{e}.\textit{g}.\xspace}

\newcommand{\etc}{\textit{etc}.\xspace}

\newcommand{\MIA}{MedIA\xspace}


\newcommand{\parggg}[1]{\phantomsection\textbf{#1}}

\newcommand{\secref}[1]{{$\S$\ref{#1}}}
\newcommand{\pgref}[1]{{(p.~\pageref{#1})}}


\newcommand{\lc}[1]{}


\newcolumntype{C}[1]{>{\centering\let\newline\\\arraybackslash\hspace{0pt}}m{#1}}


\newcommand{\cmrule}{\arrayrulecolor{black}\cmidrule(lr){2-8}\arrayrulecolor{black}}
\newcommand{\ccmrule}{\arrayrulecolor{lightgray!20}\cmidrule(lr){3-8}\arrayrulecolor{black}}
\newcommand{\ccmruleaa}{\arrayrulecolor{lightgray!20}\cmidrule(lr){3-7}\arrayrulecolor{black}}

\newcommand{\mrow}[2]{\multirow{#1}{1.5cm}{\centering #2}}



